Liapunov Multipliers and Decay of Correlations in Dynamical Systems

The essential decorrelation rate of a hyperbolic dynamical system is the decay rate of time-correlations one expects to see stably for typical observables once resonances are projected out. We define and illustrate these notions and study the conjecture that for observables in $C^1$, the essential decorrelation rate is never faster than what is dictated by the {\em smallest} unstable Liapunov multiplier.

==> baker1.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       2.00       2.05 {\rlap{0}}
\point       3.11       2.05 {\rlap{a}}
\point       5.18       2.05 {\rlap{1}}
\point       1.50       2.43 {\rlap{0}}
\point       1.50       5.61 {\rlap{1}}
\point       7.72       2.05 {\rlap{0}}
\point       7.22       3.54 {\rlap{a}}
\point      10.90       2.05 {\rlap{1}}
\point       7.22       2.43 {\rlap{0}}
\point       7.22       5.61 {\rlap{1}}
 }}


==> baker2.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       0.31       0.36 {\clap{0}}
\point       2.45       0.36 {\clap{0.5}}
\point       4.59       0.36 {\clap{1}}
\point      -0.19       0.71 {\rlap{0}}
\point      -0.19       4.99 {\rlap{1}}
\point       5.45       0.81 {\llap{$a$}}
 }}


==> baladi1.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       7.57       1.36 {\rlap{1}}
\point       1.38       1.36 {\rlap{0}}
\point       1.01       8.23 {\llap{1}}
\point       1.01       1.98 {\llap{0}}
\point       2.05       1.18 {\clap{${2\lambda^2\over1+\lambda}$}}
\point       3.40       1.18 {\clap{${1-2\lambda^2\over\lambda^2}$}}
\point       4.68       1.18 {\clap{${1-2\lambda^2\over\lambda^2}$}}
\point       6.45       1.18 {\clap{$1-{2\over\lambda^2}$}}
\point       4.3           2.1 {\clap{$x_c$}}
 }}


==> baladi2.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       7.57       1.36 {\rlap{1}}
\point       1.38       1.36 {\rlap{0}}
\point       1.01       6.24 {\llap{1}}
\point       1.01       1.98 {\llap{0}}
\point       8.20       1.48 {\rlap{$x$}}
\point       1.52       7.30 {\rlap{$h(x)$}}
\point       2.05       1.18 {\clap{${2\lambda^2\over1+\lambda}$}}
\point       3.40       1.18 {\clap{${1-2\lambda^2\over\lambda^2}$}}
\point       4.68       1.18 {\clap{${1-2\lambda^2\over\lambda^2}$}}
\point       6.45       1.18 {\clap{$1-{2\over\lambda^2}$}}
\point       2.05       1.18 {\clap{${2\lambda^2\over1+\lambda}$}}
\point       2.05       3.09 {\clap{${2\lambda^2\over N}$}}
\point       3.40       3.89 {\clap{${\lambda(1+\lambda)\over N}$}}
\point       4.68       3.89 {\clap{${\lambda(1+\lambda)\over N}$}}
\point       6.45       4.18 {\clap{${2(1+\lambda^2)\over N}$}}
 }}


==> baladi3.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
 }}


==> baladi4.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point      -0.51       4.50 {\rlap{$ 0$}                   }
\point       0.28       4.50 {\rlap{$ 1$}                   }
\point       1.08       4.50 {\rlap{$ 2$}                   }
\point       1.87       4.50 {\rlap{$ 3$}                   }
\point       2.66       4.50 {\rlap{$ 4$}                   }
\point       3.46       4.50 {\rlap{$ 5$}                   }
\point       4.25       4.50 {\rlap{$ 6$}                   }
\point       5.04       4.50 {\rlap{$ 7$}                   }
\point       5.84       4.50 {\rlap{$ 8$}                   }
\point       6.63       4.50 {\rlap{$ 9$}                   }
\point       7.42       4.50 {\rlap{$10$}                   }
\point       8.22       4.50 {\rlap{$11$}                   }
\point       9.01       4.50 {\rlap{$12$}                   }
\point       9.61       5.20 {\clap{${k}$}}
 }}



==> baladi5.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point      -0.31       4.35 {\clap{$ 0$}                   }
\point       0.48       4.35 {\clap{$ 1$}                   }
\point       1.28       4.35 {\clap{$ 2$}                   }
\point       2.07       4.35 {\clap{$ 3$}                   }
\point       2.86       4.35 {\clap{$ 4$}                   }
\point       3.66       4.35 {\clap{$ 5$}                   }
\point       4.45       4.35 {\clap{$ 6$}                   }
\point       5.24       4.35 {\clap{$ 7$}                   }
\point       6.04       4.35 {\clap{$ 8$}                   }
\point       6.83       4.35 {\clap{$ 9$}                   }
\point       7.62       4.35 {\clap{$10$}                   }
\point       8.42       4.35 {\clap{$11$}                   }
\point       9.21       4.35 {\clap{$12$}                   }
\point       9.85       5.20 {\clap{${k}$}}
 }}


==> www.tex <==
\def\fact{8}
\newdimen\xxxx
\newdimen\yyyy
 \def\point#1 #2 #3 {\xxxx=#1 truecm\relax\multiply\xxxx by
 \fact\divide\xxxx by 10 %
\yyyy=#2 truecm\relax\multiply \yyyy by \fact \divide \yyyy by 10 %
\rlap{\kern \xxxx 
 \raise \yyyy  \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       12 9.4  {${W}^u$}
\point       5.8 -0.6  {${\cal W}^s$}
\point       3.8 0.0  {${W}^s$}
\point       16.6 7.7  {${\cal W}^u$}
\point       14.6 5.8  {${\cal W}^{u_{\rm min}}$}
\point       12.4 4.4  {${w = W^{u_{\rm min}}}$}
\point 4.2 1.9 {$x$}
\point 6.3 2.6 {$\vec t_{x}$}
%\point 9.2 3.5 {$\vec y_w(s)$}
%\point 11.7 4.2 {$x(w,s)$}
}}

